Large-Scale In-Game Outcome Forecasting for Match, Team and Players in Football using an Axial Transformer Neural Network

Football (soccer) is a sport that is characterised by complex game play, where players perform a variety of actions, such as passes, shots, tackles, fouls, in order to score goals, and ultimately win matches. Accurately forecasting the total number of each action that each player will complete during a match is desirable for a variety of applications, including tactical decision-making, sports betting, and for television broadcast commentary and analysis. Such predictions must consider the game state, the ability and skill of the players in both teams, the interactions between the players, and the temporal dynamics of the game as it develops. In this paper, we present a transformer-based neural network that jointly and recurrently predicts the expected totals for thirteen individual actions at multiple time-steps during the match, and where predictions are made for each individual player, each team and at the game-level. The neural network is based on an \emph{axial transformer} that efficiently captures the temporal dynamics as the game progresses, and the interactions between the players at each time-step. We present a novel axial transformer design that we show is equivalent to a regular sequential transformer, and the design performs well experimentally. We show empirically that the model can make consistent and reliable predictions, and efficiently makes $\sim$75,000 live predictions at low latency for each game.

==> tables/test-logprob-by-target.tex <==
\begin{table}
\caption{Abalation test results by team event.}
\label{tbl:test-results-team}
\begin{tabular}{lrrrrrrrrrr}
\toprule
metric & \multicolumn{5}{r}{Logprob} & \multicolumn{5}{r}{Calibration error} \\
model & Ours & Ours wo spatial & Ours wo temporal & Ours wo pregame & Ours with stacked & Ours & Ours wo spatial & Ours wo temporal & Ours wo pregame & Ours with stacked \\
target &  &  &  &  &  &  &  &  &  &  \\
\midrule
Goals & -0.928 & -0.961 & -0.941 & -0.943 & -0.927 & 0.020 & 0.033 & 0.027 & 0.018 & 0.016 \\
Assists & -0.758 & -0.781 & -0.768 & -0.769 & -0.757 & 0.017 & 0.029 & 0.028 & 0.015 & 0.015 \\
Shots & -2.226 & -2.442 & -2.290 & -2.287 & -2.229 & 0.022 & 0.051 & 0.033 & 0.034 & 0.022 \\
Shots on target & -1.547 & -1.610 & -1.556 & -1.565 & -1.543 & 0.012 & 0.027 & 0.018 & 0.025 & 0.008 \\
Corners & -1.655 & -1.750 & -1.692 & -1.683 & -1.658 & 0.027 & 0.041 & 0.036 & 0.034 & 0.025 \\
Attempted passes & -8.082 & -13.898 & -9.288 & -9.351 & -8.177 & 0.025 & 0.033 & 0.036 & 0.033 & 0.025 \\
Accurate passes & -8.715 & -13.725 & -10.186 & -10.218 & -8.843 & 0.030 & 0.038 & 0.040 & 0.038 & 0.030 \\
Tackles & -2.301 & -2.474 & -2.308 & -2.310 & -2.315 & 0.016 & 0.042 & 0.023 & 0.024 & 0.016 \\
Fouls & -2.016 & -2.167 & -2.035 & -2.075 & -2.022 & 0.012 & 0.022 & 0.021 & 0.023 & 0.009 \\
Yellow cards & -1.287 & -1.336 & -1.300 & -1.307 & -1.289 & 0.015 & 0.024 & 0.009 & 0.020 & 0.014 \\
Red cards & -0.020 & -0.228 & -0.217 & -0.227 & -0.020 & 0.002 & 0.016 & 0.007 & 0.013 & 0.002 \\
Own goals & -0.088 & -0.089 & -0.090 & -0.089 & -0.088 & 0.004 & 0.003 & 0.002 & 0.005 & 0.003 \\
\bottomrule
\end{tabular}
\end{table}

\begin{table}
\caption{Abalation test results by player event.}
\label{tbl:test-results-player}
\begin{tabular}{lrrrrrrrrrr}
\toprule
metric & \multicolumn{5}{r}{Logprob} & \multicolumn{5}{r}{Calibration error} \\
model & Ours & Ours wo spatial & Ours wo temporal & Ours wo pregame & Ours with stacked & Ours & Ours wo spatial & Ours wo temporal & Ours wo pregame & Ours with stacked \\
target &  &  &  &  &  &  &  &  &  &  \\
\midrule
Goals & -0.111 & -0.114 & -0.124 & -0.124 & -0.112 & 0.002 & 0.013 & 0.004 & 0.014 & 0.002 \\
Assists & -0.088 & -0.090 & -0.098 & -0.094 & -0.089 & 0.001 & 0.002 & 0.004 & 0.001 & 0.001 \\
Shots & -0.515 & -0.532 & -0.575 & -0.597 & -0.520 & 0.021 & 0.022 & 0.028 & 0.044 & 0.021 \\
Shots on target & -0.260 & -0.266 & -0.289 & -0.296 & -0.262 & 0.016 & 0.018 & 0.011 & 0.031 & 0.015 \\
Corners & -0.289 & -0.299 & -0.323 & -0.320 & -0.292 & 0.019 & 0.020 & 0.013 & 0.030 & 0.017 \\
Attempted passes & -3.039 & -3.333 & -3.501 & -3.735 & -3.062 & 0.074 & 0.093 & 0.093 & 0.102 & 0.076 \\
Accurate passes & -2.765 & -3.002 & -3.199 & -3.403 & -2.781 & 0.075 & 0.094 & 0.096 & 0.109 & 0.078 \\
Tackles & -0.608 & -0.620 & -0.674 & -0.661 & -0.614 & 0.027 & 0.025 & 0.029 & 0.028 & 0.024 \\
Fouls & -0.517 & -0.530 & -0.569 & -0.558 & -0.524 & 0.018 & 0.023 & 0.021 & 0.028 & 0.020 \\
Yellow cards & -0.202 & -0.209 & -0.220 & -0.211 & -0.203 & 0.019 & 0.020 & 0.004 & 0.023 & 0.019 \\
Red cards & -0.018 & -0.019 & -0.020 & -0.019 & -0.019 & 0.000 & 0.000 & 0.003 & 0.000 & 0.000 \\
Own goals & -0.006 & -0.007 & -0.007 & -0.007 & -0.006 & 0.000 & 0.000 & 0.001 & 0.000 & 0.000 \\
\bottomrule
\end{tabular}
\end{table}

\begin{table}
\caption{Generalization metrics.}
\label{tbl:generalization-results}
\begin{tabular}{lrrr}
\toprule
 & Val logprob & Test logprob & Rel difference \\
target &  &  &  \\
\midrule
Game outcome & -0.666 & -0.673 & 1.009 \\
Goals & -0.113 & -0.111 & 0.983 \\
Assists & -0.090 & -0.088 & 0.983 \\
Shots & -0.515 & -0.515 & 0.998 \\
Shots on target & -0.263 & -0.260 & 0.991 \\
Corners & -0.293 & -0.289 & 0.989 \\
Attempted passes & -2.934 & -3.039 & 1.036 \\
Accurate passes & -2.642 & -2.765 & 1.047 \\
Tackles & -0.599 & -0.608 & 1.015 \\
Fouls & -0.540 & -0.517 & 0.957 \\
Yellow cards & -0.197 & -0.202 & 1.021 \\
Red cards & -0.021 & -0.018 & 0.871 \\
Own goals & -0.006 & -0.006 & 1.012 \\
\bottomrule
\end{tabular}
\end{table}

